Planck intermediate results. VII. Statistical properties of infrared and radio extragalactic sources from the Planck Early Release Compact Source Catalogue at frequencies between 100 and 857 GHz

(abridged for arXiv) We make use of the Planck all-sky survey to derive number counts and spectral indices of extragalactic sources -- infrared and radio sources -- from the Planck Early Catalogue (ERCSC) at 100 to 857GHz. Our sample contains, after the 80% completeness cut, between 122 and 452 and sources, with flux densities above 0.3 and 1.9Jy at 100 and 857GHz, over about 31 to 40% of the sky. Using Planck HFI, all the sources have been classified as either dust-dominated or synchrotron-dominated on the basis of their spectral energy distributions (SED). Our sample is thus complete, flux-limited and color-selected to differentiate between the two populations. We find an approximately equal number of synchrotron and dusty sources between 217 and 353GHz; at 353GHz or higher (or 217GHz and lower) frequencies, the number is dominated by dusty (synchrotron) sources, as expected. For most of the sources, the spectral indices are also derived. We provide for the first time counts of bright sources from 353 to 857GHz and the contributions from dusty and synchrotron sources at all HFI frequencies in the key spectral range where these spectra are crossing. The observed counts are in the Euclidean regime. The number counts are compared to previously published data (earlier Planck, Herschel, BLAST, SCUBA, LABOCA, SPT, and ACT) and models taking into account both radio or infrared galaxies. We derive the multi-frequency Euclidean level and compare it to WMAP, Spitzer and IRAS results. The submillimetre number counts are not well reproduced by current evolution models of dusty galaxies, whereas the millimetre part appears reasonably well fitted by the most recent model for synchrotron-dominated sources. Finally we provide estimates of the local luminosity density of dusty galaxies, providing the first such measurements at 545 and 857GHz.

==> table_number_counts_highfreq.tex <==
%
% Table NUMBER COUNTS
%---------------------------------------------------------------
\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{\Planck\ number counts at 353, 545 and 857 GHz.}                          % Caption goes here.
\label{tab:number_counts_highfreq}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
  \newdimen\digitwidth 
  \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{ # & # & # & # & # & # & # & # \cr                        % Template goes here.
\noalign{\doubleline}
                        % Table headings go here.
    $\left < S_{\nu} \right >$  &  $S_{\nu}$ range  & $dN/dS_{857}S_{857}^{2.5}$ & $N({>}S_{857})$ & $dN/dS_{545}S_{545}^{2.5}$ & $N({>}S_{545})$ & $dN/dS_{353}S_{353}^{2.5}$ & $N({>}S_{353})$   \cr
    $[$Jy$]$ &   [Jy] &    [Jy$^{1.5}$\,sr$^{-1}$] & [sr$^{-1}$] &[Jy$^{1.5}$\,sr$^{-1}]$ &[sr$^{-1}$]&[Jy$^{1.5}$\,sr$^{-1}$] &[sr$^{-1}$]  \cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
                        % Body of table goes here.
  0.631 &   0.480 --   0.762 &  --  &  --  &  --  &  --  & $   30.6 \pm   3.7 $ & $   50.1 \pm   3.3 $ \cr 
  1.000 &   0.762 --   1.207 &  --  &  --  &  --  &  --  & $   26.4 \pm   4.0 $ & $   21.0 \pm   2.1 $ \cr 
  1.585 &   1.207 --   1.913 &  --  &  --  & $  131.4 \pm  21.4 $ & $   60.3 \pm   4.1 $ & $   17.6 \pm   4.1 $ & $    8.4 \pm   1.3 $ \cr 
  2.512 &   1.913 --   3.032 & $  466.2 \pm  70.5 $ & $  127.7 \pm   6.0 $ & $  104.6 \pm  20.4 $ & $   28.9 \pm   2.7 $ & $   18.3 \pm   5.7 $ & $    4.2 \pm   0.9 $ \cr 
  3.981 &   3.032 --   4.805 & $  613.6 \pm  96.6 $ & $   71.8 \pm   4.4 $ & $  160.2 \pm  33.8 $ & $   16.3 \pm   2.1 $ & $   23.3 \pm   9.0 $ & $    2.0 \pm   0.6 $ \cr 
  6.310 &   4.805 --   7.615 & $  573.4 \pm 103.4 $ & $   35.0 \pm   3.0 $ & $  129.4 \pm  37.5 $ & $    6.7 \pm   1.3 $ &  --  &  --  \cr 
 10.000 &   7.615 --  12.069 & $  755.2 \pm 150.3 $ & $   17.7 \pm   2.1 $ & $  119.5 \pm  47.8 $ & $    2.8 \pm   0.9 $ & $   13.2 \pm  13.3 $ & $    0.6 \pm   0.3 $ \cr 
 15.849 &  12.069 --  22.801 & $  837.1 \pm 200.5 $ & $    6.3 \pm   1.3 $ & $  136.2 \pm  70.4 $ & $    1.0 \pm   0.5 $ & $   52.9 \pm  37.6 $ & $    0.4 \pm   0.3 $ \cr 
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
%\tablenote a Footnote a.\par
%\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.
%---------------------------------------------------------------
% written by make_tables_number_counts_ercsc.pro on Thu Jun  7 17:23:56 2012


==> table_number_counts_highfreq_dusty.tex <==
%
% Table NUMBER COUNTS
%---------------------------------------------------------------
\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{\Planck\ number counts of dusty galaxies (only) between 217 and 857 GHz.}                          % Caption goes here.
\label{tab:number_counts_dusty}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
  \newdimen\digitwidth 
  \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{ # & # & # & # & # & # & # & # \cr                        % Template goes here.
\noalign{\doubleline}
                        % Table headings go here.
    $\left < S_{\nu} \right >$  &  $S_{\nu}$ range & $dN/dS_{857}S_{857}^{2.5}$ & $dN/dS_{545}S_{545}^{2.5}$ &  $dN/dS_{353}S_{353}^{2.5}$ &  $dN/dS_{217}S_{217}^{2.5}$  \cr
     $[$Jy$]$ &   [Jy] &    [Jy$^{1.5}$\,sr$^{-1}$] & [Jy$^{1.5}$\,sr$^{-1}$] &[Jy$^{1.5}$\,sr$^{-1}$] &[Jy$^{1.5}$\,sr$^{-1}$]   \cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
                        % Body of table goes here.
  0.398 &   0.303 --   0.480 &  --  &  --  &  --  & $    3.2 \pm   0.7 $ \cr 
  0.631 &   0.480 --   0.762 &  --  &  --  & $   23.6 \pm   3.1 $ & $    2.3 \pm   0.8 $ \cr 
  1.000 &   0.762 --   1.207 &  --  &  -- & $   18.5 \pm   3.2 $ & $    1.8 \pm   0.9 $ \cr 
  1.585 &   1.207 --   1.913 &  --  & $  129.0 \pm  21.1 $ & $   12.5 \pm   3.4 $ &  --  \cr 
  2.512 &   1.913 --   3.032 & $  463.6 \pm  70.2 $ & $  100.3 \pm  19.8 $ & $   11.7 \pm   4.5 $ & $    1.7 \pm   1.7 $ \cr 
  3.981 &   3.032 --   4.805 & $  609.0 \pm  96.0 $ & $  151.5 \pm  32.5 $ & $   13.3 \pm   6.7 $ &  --  \cr 
  6.310 &   4.805 --   7.615 & $  573.4 \pm 103.4 $ & $  129.4 \pm  37.5 $ &  --  &  --  \cr 
 10.000 &   7.615 --  12.069 & $  755.2 \pm 150.3 $ & $  119.5 \pm  47.8 $ & $   13.2 \pm  13.3 $ &  --  \cr 
 15.849 &  12.069 --  22.801 & $  837.1 \pm 200.5 $ & $  136.2 \pm  70.4 $ & $   26.4 \pm  26.5 $ &  --  \cr 
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
%\tablenote a Footnote a.\par
%\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.
%---------------------------------------------------------------
% written by make_tables_number_counts_ercsc.pro on Thu Jun  7 17:23:56 2012


==> table_number_counts_lowfreq.tex <==
%
% Table NUMBER COUNTS
%---------------------------------------------------------------
\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{\Planck\ number counts at 100, 143 and 217 GHz.}                          % Caption goes here.
\label{tab:number_counts_lowfreq}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
  \newdimen\digitwidth 
  \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{ # & # & # & # & # & # & # & # \cr                        % Template goes here.
\noalign{\doubleline}
                        % Table headings go here.
    $\left < S_{\nu} \right >$  &  $S_{\nu}$ range  & $dN/dS_{217}S_{217}^{2.5}$ & $N({>}S_{217}$) & $dN/dS_{143}S_{143}^{2.5}$ & $N({>}S_{143})$ & $dN/dS_{100}S_{100}^{2.5}$ & $N({>}S_{100})$   \cr
    $[$Jy$]$ &   [Jy] &    [Jy$^{1.5}$\,sr$^{-1}$] & [sr$^{-1}$] &[Jy$^{1.5}$\,sr$^{-1}]$ &[sr$^{-1}$]&[Jy$^{1.5}$\,sr$^{-1}$] &[sr$^{-1}$]  \cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
                        % Body of table goes here.
  0.398 &   0.303 --   0.480 & $   16.5 \pm   2.0 $ & $   54.3 \pm  3.54 $ & $    8.5 \pm   1.1 $ & $   44.3 \pm  2.95 $ &  --  &  --  \cr 
  0.631 &   0.480 --   0.762 & $   11.5 \pm   1.9 $ & $   23.0 \pm  2.21 $ & $   13.7 \pm   2.1 $ & $   28.1 \pm  2.46 $ & $   21.9 \pm   3.0 $ & $   43.7 \pm  3.14 $ \cr 
  1.000 &   0.762 --   1.207 & $   14.6 \pm   2.8 $ & $   12.0 \pm  1.58 $ & $   17.4 \pm   3.1 $ & $   15.0 \pm  1.77 $ & $   29.1 \pm   4.4 $ & $   22.9 \pm  2.22 $ \cr 
  1.585 &   1.207 --   1.913 & $   13.6 \pm   3.6 $ & $    5.1 \pm  1.01 $ & $   15.4 \pm   3.8 $ & $    6.7 \pm  1.17 $ & $   18.8 \pm   4.3 $ & $    9.1 \pm  1.35 $ \cr 
  2.512 &   1.913 --   3.032 & $    6.8 \pm   3.4 $ & $    1.8 \pm  0.61 $ & $   13.6 \pm   5.0 $ & $    3.1 \pm  0.79 $ & $   23.2 \pm   6.5 $ & $    4.6 \pm  0.95 $ \cr 
  3.981 &   3.032 --   4.805 & $   10.1 \pm   5.9 $ & $    1.0 \pm  0.45 $ & $   13.6 \pm   6.9 $ & $    1.4 \pm  0.54 $ & $   16.5 \pm   7.5 $ & $    1.8 \pm  0.59 $ \cr 
  6.310 &   4.805 --   7.615 & $   13.5 \pm   9.6 $ & $    0.4 \pm  0.29 $ & $   13.6 \pm   9.7 $ & $    0.6 \pm  0.35 $ & $   13.2 \pm   9.4 $ & $    0.8 \pm  0.40 $ \cr 
 10.000 &   7.615 --  12.069 &  --  &  --  & $   13.6 \pm  13.6 $ & $    0.2 \pm  0.20 $ & $   26.3 \pm  18.7 $ & $    0.4 \pm  0.28 $ \cr 
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
%\tablenote a Footnote a.\par
%\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.
%---------------------------------------------------------------
% written by make_tables_number_counts_ercsc.pro on Thu Jun  7 17:23:56 2012


==> table_number_counts_lowfreq_synch.tex <==
%
% Table NUMBER COUNTS
%---------------------------------------------------------------
\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{\Planck\ number counts of (only) synchrotron galaxies between 100 and 857 GHz.}                          % Caption goes here.
\label{tab:number_counts_synch}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
  \newdimen\digitwidth 
  \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{ # & # & # & # & # & # & # & # \cr                        % Template goes here.
\noalign{\doubleline}
                        % Table headings go here.
    $\left < S_{\nu} \right >$  &  $S_{\nu}$ range &  $dN/dS_{857}S_{857}^{2.5}$ &  $dN/dS_{545}S_{545}^{2.5}$ &  $dN/dS_{353}S_{353}^{2.5}$ &  $dN/dS_{217}S_{217}^{2.5}$ &  $dN/dS_{143}S_{143}^{2.5}$  & $dN/dS_{100}S_{100}^{2.5}$  \cr
     $[$Jy$]$ &   [Jy] &    [Jy$^{1.5}$\,sr$^{-1}$] & [Jy$^{1.5}$\,sr$^{-1}$] & [Jy$^{1.5}$\,sr$^{-1}$] &[Jy$^{1.5}$\,sr$^{-1}$] &[Jy$^{1.5}$\,sr$^{-1}$] &[Jy$^{1.5}$\,sr$^{-1}$]  \cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
                        % Body of table goes here.
  0.398 &   0.303 --   0.480 &  --  &  --  &  --  & $   13.3 \pm   1.7 $ & $    8.5 \pm   1.1 $ &  --  \cr 
  0.631 &   0.480 --   0.762 &  --  &  --  & $    7.0 \pm   1.4 $ & $    9.2 \pm   1.6 $ & $   13.5 \pm   2.1 $ & $   21.9 \pm   3.0 $ \cr 
  1.000 &   0.762 --   1.207 &  --  &  --  & $    7.9 \pm   2.0 $ & $   12.8 \pm   2.6 $ & $   16.9 \pm   3.1 $ & $   28.6 \pm   4.3 $ \cr 
  1.585 &   1.207 --   1.913 &  --  & $    2.4 \pm   1.7 $ & $    5.0 \pm   2.1 $ & $   13.6 \pm   3.6 $ & $   15.4 \pm   3.8 $ & $   18.8 \pm   4.3 $ \cr 
  2.512 &   1.913 --   3.032 & $    2.6 \pm   2.6 $ & $    4.3 \pm   3.1 $ & $    6.7 \pm   3.4 $ & $    5.1 \pm   3.0 $ & $   13.6 \pm   5.0 $ & $   23.2 \pm   6.5 $ \cr 
  3.981 &   3.032 --   4.805 & $    4.5 \pm   4.6 $ & $    8.7 \pm   6.2 $ & $   10.0 \pm   5.8 $ & $   10.1 \pm   5.9 $ & $   13.6 \pm   6.9 $ & $   16.5 \pm   7.5 $ \cr 
  6.310 &   4.805 --   7.615 &  --  &  --  &  --  & $   13.5 \pm   9.6 $ & $   13.6 \pm   9.7 $ & $   13.2 \pm   9.4 $ \cr 
 10.000 &   7.615 --  12.069 &  --  &  --  &  --  &  --  & $   13.6 \pm  13.6 $ & $   26.3 \pm  18.7 $ \cr 
 15.849 &  12.069 --  22.801 &  --  &  --  & $   26.4 \pm  26.5 $ &  --  &  --  &  --  \cr 
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
%\tablenote a Footnote a.\par
%\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.
%---------------------------------------------------------------
% written by make_tables_number_counts_ercsc.pro on Thu Jun  7 17:23:56 2012


==> table_numbers_planck_numbercounts.tex <==
%
% Table NUMBER of SOURCES by ZONE
%---------------------------------------------------------------
\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Number of extragalactic ERCSC sources actually used in the number counts: deep -- medium -- shallow, with the numbers of unidentified sources after the slash.}                          % Caption goes here.
\label{tab:numbers}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
  \newdimen\digitwidth 
  \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{ # & # & # & # & # & # & # & # \cr                        % Template goes here.
\noalign{\doubleline}
                        % Table headings go here.
    $\left < S_{\nu} \right >$  &  $S_{\nu}$ range  & $857$\,GHz & $545$\,GHz & $353$\,GHz & $217$\,GHz & $143$\,GHz & $100$\,GHz  \cr
     $[$Jy$]$          &   [Jy]              &       &       &       &       &       &   \cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
                        % Body of table goes here.
  0.398 &   0.303 --   0.480 &  0  &  0  &  0  &  7/0 -- 28/1  -- 92/9  &  3/0 -- 12/0  -- 81/1  &  0  \cr 
  0.631 &   0.480 --   0.762 &  0  &  0  &  8/0 -- 31/4  -- 83/14  &  3/0 -- 13/1  -- 34/2  &  2/0 -- 13/0  -- 43/0  &  4/0 -- 15/0  -- 68/3  \cr 
  1.000 &   0.762 --   1.207 &  0  &  0  &  4/0 -- 18/2  -- 38/7  &  4/0 -- 8/0  -- 21/1  &  4/0 -- 10/0  -- 25/0  &  4/0 -- 11/0  -- 47/1  \cr 
  1.585 &   1.207 --   1.913 &  0  &  5/0 -- 26/6  -- 78/9  &  1/1 -- 6/0  -- 14/0  &  1/0 -- 4/0  -- 11/0  &  2/0 -- 4/0  -- 12/0  &  2/0 -- 7/0  -- 13/0  \cr 
  2.512 &   1.913 --   3.032 &  11/0 -- 31/1  -- 139/4  &  0/0 -- 20/1  -- 28/1  &  1/0 -- 2/0  -- 8/0  &  0/0 -- 1/0  -- 3/0  &  0/0 -- 3/0  -- 5/0  &  0/0 -- 3/0  -- 11/0  \cr 
  3.981 &   3.032 --   4.805 &  7/0 -- 33/2  -- 95/4  &  1/0 -- 16/1  -- 20/1  &  0/0 -- 1/0  -- 6/0  &  0/0 -- 2/0  -- 1/0  &  0/0 -- 1/0  -- 3/0  &  0/0 -- 2/0  -- 3/0  \cr 
  6.310 &   4.805 --   7.615 &  3/0 -- 22/2  -- 41/7  &  1/0 -- 6/0  -- 8/1  &  0  &  0/0 -- 1/0  -- 1/0  &  0/0 -- 1/0  -- 1/0  &  0/0 -- 0/0  -- 2/0  \cr 
 10.000 &   7.615 --  12.069 &  2/0 -- 20/1  -- 23/1  &  1/0 -- 1/0  -- 5/0  &  0/0 -- 1/0  -- 0/0  &  0  &  0/0 -- 0/0  -- 1/0  &  0/0 -- 1/0  -- 1/0  \cr 
 15.849 &  12.069 --  22.801 &  1/0 -- 9/0  -- 15/0  &  0/0 -- 0/0  -- 4/0  &  0/0 -- 0/0  -- 2/0  &  0  &  0  &  0  \cr 
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
%\tablenote a Footnote a.\par
%\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.
%---------------------------------------------------------------
% written by make_tables_number_counts_ercsc.pro on Thu Jun  7 17:23:56 2012


==> table_source_identifications.tex <==
%
% Table source identifications
%---------------------------------------------------------------
\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Percentage of \Planck\ source identifications using the SIMBAD and NED databases (with the number of sources in parentheses).}       % Caption goes here.
\label{tab:ids}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
  \newdimen\digitwidth 
  \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{ # & # & # & # & # & #  \cr                        % Template goes here.
\noalign{\doubleline}
                        % Table headings go here.
    $\nu$  & Extragalactic  & Galactic    & Galactic       & Unidentified    & Total \cr
       $[$GHz$]$   & Secure \% (No.) & Unsecure \% (No.) & Secure \% (No.) &  \% (No.) & \% (No.) \cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
                        % Body of table goes here.
857 deep &  91.2 (73) &  2.5 (2) &  1.2 (1) &  5.0 (4) & 100 (80)  \cr
857 medium &  95.5 (255) &  1.9 (5) &  0.0 (0) &  2.6 (7) & 100 (267)  \cr
857 shallow &  94.6 (697) &  1.6 (12) &  0.8 (6) &  3.0 (22) & 100 (737)  \cr
\noalign{\vskip 1pt\hrule\vskip 1pt} \cr
545 deep &  76.5 (39) &  7.8 (4) &  2.0 (1) & 13.7 (7) & 100 (51)  \cr
545 medium &  91.1 (143) &  2.5 (4) &  0.0 (0) &  6.4 (10) & 100 (157)  \cr
545 shallow &  91.8 (301) &  2.1 (7) &  0.9 (3) &  5.2 (17) & 100 (328)  \cr
\noalign{\vskip 1pt\hrule\vskip 1pt} \cr
353 deep &  81.6 (31) &  2.6 (1) &  5.3 (2) & 10.5 (4) & 100 (38)  \cr
353 medium &  87.0 (94) &  0.9 (1) &  2.8 (3) &  9.3 (10) & 100 (108)  \cr
353 shallow &  78.0 (170) &  4.6 (10) &  4.6 (10) & 12.8 (28) & 100 (218)  \cr
\noalign{\vskip 1pt\hrule\vskip 1pt} \cr
217 deep &  77.3 (17) &  0.0 (0) & 22.7 (5) &  0.0 (0) & 100 (22)  \cr
217 medium &  92.5 (62) &  1.5 (1) &  1.5 (1) &  4.5 (3) & 100 (67)  \cr
217 shallow &  88.5 (170) &  0.5 (1) &  4.2 (8) &  6.8 (13) & 100 (192)  \cr
\noalign{\vskip 1pt\hrule\vskip 1pt} \cr
143 deep &  86.7 (13) &  0.0 (0) & 13.3 (2) &  0.0 (0) & 100 (15)  \cr
143 medium & 100.0 (48) &  0.0 (0) &  0.0 (0) &  0.0 (0) & 100 (48)  \cr
143 shallow &  96.8 (182) &  0.5 (1) &  1.6 (3) &  1.1 (2) & 100 (188)  \cr
\noalign{\vskip 1pt\hrule\vskip 1pt} \cr
100 deep &  77.8 (14) &  0.0 (0) & 22.2 (4) &  0.0 (0) & 100 (18)  \cr
100 medium & 100.0 (45) &  0.0 (0) &  0.0 (0) &  0.0 (0) & 100 (45)  \cr
100 shallow &  93.9 (154) &  0.0 (0) &  3.7 (6) &  2.4 (4) & 100 (164)  \cr
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
%\tablenote a Footnote a.\par
%\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.
%---------------------------------------------------------------
% written by make_tables_number_counts_ercsc.pro on Thu Jun  7 17:23:56 2012


==> table_source_zone_stat_planck_numbercounts.tex <==
%
% Table stats on sources and zones
%---------------------------------------------------------------
\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{Number of extragalactic ERCSC sources in our sample prior to the completeness cut (and after the completeness cut in parentheses), together with the surface area of the zones.}                          % Caption goes here.
\label{tab:sourcenumber}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
  \newdimen\digitwidth 
  \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{ # & # & #  & #  & #  & #  & #  & #  & # \cr                        % Template goes here.
\noalign{\doubleline}
                        % Table headings go here.
     $\nu$  & number  & number  & number  & total source & surface area & surface area & surface area & total surface \cr
      $[$GHz$]$   & deep    & medium &  shallow &     number             &   deep  &  medium  & shallow & [deg$^2$]\cr
\noalign{\vskip 3pt\hrule\vskip 5pt}
                        % Body of table goes here.
857 & 77 (24) & 262 (115) & 719 (313) & 1058 (452) &   880 &  2288 &  9800 & 12969\cr
545 & 46 (8) & 153 (69) & 318 (143) & 517 (220) &   874 &  2324 &  9551 & 12749\cr
353 & 35 (14) & 104 (59) & 198 (151) & 337 (224) &  1086 &  2971 & 12373 & 16431\cr
217 & 17 (15) & 65 (57) & 183 (71) & 265 (143) &  1104 &  3169 & 11900 & 16174\cr
143 & 13 (8) & 48 (44) & 184 (90) & 245 (142) &  1111 &  2972 & 11977 & 16061\cr
100 & 14 (6) & 45 (39) & 158 (77) & 217 (122) &  1072 &  2870 & 12611 & 16554\cr
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
%\tablenote a Footnote a.\par
%\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.
%---------------------------------------------------------------
% written by make_tables_number_counts_ercsc.pro on Thu Jun  7 17:23:56 2012

